Learning Dynamic Embeddings from Temporal Interactions

Modeling a sequence of interactions between users and items (e.g., products, posts, or courses) is crucial in domains such as e-commerce, social networking, and education to predict future interactions. Representation learning presents an attractive solution to model the dynamic evolution of user and item properties, where each user/item can be embedded in a euclidean space and its evolution can be modeled by dynamic changes in embedding. However, existing embedding methods either generate static embeddings, treat users and items independently, or are not scalable. Here we present JODIE, a coupled recurrent model to jointly learn the dynamic embeddings of users and items from a sequence of user-item interactions. JODIE has three components. First, the update component updates the user and item embedding from each interaction using their previous embeddings with the two mutually-recursive Recurrent Neural Networks. Second, a novel projection component is trained to forecast the embedding of users at any future time. Finally, the prediction component directly predicts the embedding of the item in a future interaction. For models that learn from a sequence of interactions, traditional training data batching cannot be done due to complex user-user dependencies. Therefore, we present a novel batching algorithm called t-Batch that generates time-consistent batches of training data that can run in parallel, giving massive speed-up. We conduct six experiments on two prediction tasks---future interaction prediction and state change prediction---using four real-world datasets. We show that JODIE outperforms six state-of-the-art algorithms in these tasks by up to 22.4%. Moreover, we show that JODIE is highly scalable and up to 9.2x faster than comparable models. As an additional experiment, we illustrate that JODIE can predict student drop-out from courses five interactions in advance.

==> 045analysis.tex <==
% !TEX root = paper-interactions.tex

\section{Analysis of the model}
\label{sec:analysis}

Here we analyze the usefulness of our \method\ model 


Further, in Figure~\ref{}, we show that the prediction made by \method\ is effective in early prediction of change in state. 

This is useful in 


We show that the prediction probability score of our model steadily increases as a student gets closer to dropping out. 

This illustrates that our model is effective in learning early signs of maliciousness/state change, and can potentially be used as an early-warning system.


Here we analyze our model. 


\begin{enumerate}
\item Exogenous effects: When an item is popular, its likelihood of prediction increases; IGNORE
\item Trajectory visualization or clustering 
\item Final embedding clustering
\end{enumerate}

% illustrate that different predictions are made at different times; move to experiments 
In Figure~\ref{} we illustrate the predictions made by our model for one user at various times in the future. 
We see that our model predicts that the user with interact with an item in the short term, while another item when more time has passed. 
% This would be a great example to show the effect of external events. 
\srijan{add a figure showing that the prediction changes in 1. short term vs long term and 2. due to external event (when an item is popular, then its predicted ranking increases).}


\textbf{}
Here we show that the 



